Merging automatic differentiation and the adjoint method for photonic inverse design

Optimizing shapes and topology of physical devices is crucial for both scientific and technological advancements, given its wide-ranging implications across numerous industries and research areas. Innovations in shape and topology optimization have been seen across a wide range of fields, notably structural mechanics, fluid mechanics, and photonics. Gradient-based inverse design techniques have been particularly successful for photonic and optical problems, resulting in integrated, miniaturized hardware that has set new standards in device performance. To calculate the gradients, there are typically two approaches: implementing specialized solvers using automatic differentiation or deriving analytical solutions for gradient calculation and adjoint sources by hand. In this work, we propose a middle ground and present a hybrid approach that leverages and enables the benefits of automatic differentiation and machine learning frameworks for handling gradient derivation while using existing, proven solvers for numerical solutions. Utilizing the adjoint method, we turn existing numerical solvers differentiable and seamlessly integrate them into an automatic differentiation framework. Further, this enables users to integrate the optimization environment with machine learning applications which could lead to better photonic design workflows. We illustrate the approach through two distinct examples: optimizing the Purcell factor of a magnetic dipole in the vicinity of an optical nanocavity and enhancing the light extraction efficiency of a {\textmu}LED.

==> 2_adjoint_method.tex <==
% Gradient-based optimization is a powerful technique for finding the optimal solution to complex problems by iteratively updating the parameters of the target function. One of the critical components in gradient-based optimization is the efficient computation of gradients, which can be achieved using the chain rule.

% \subsection{Gradient-based optimization and the chain rule}

% Consider a scalar function $f(\boldsymbol{x})$, where $\boldsymbol{x} \in \mathbb{R}^n$ is a vector of parameters. The gradient of $f$ with respect to $\boldsymbol{x}$ is given by:

% \begin{equation}
% \nabla f = \left( \frac{\partial f}{\partial x_1}, \frac{\partial f}{\partial x_2}, \dots, \frac{\partial f}{\partial x_n} \right)^T.
% \end{equation}

% To compute the gradient, we can use the chain rule, which states that for a composite function $f(g(\boldsymbol{x}))$, the derivative with respect to $\boldsymbol{x}$ is given by:

% \begin{equation}
% \frac{df(g(\boldsymbol{x}))}{dx_i} = \frac{df(g)}{dg} \frac{dg(\boldsymbol{x})}{dx_i}, \quad i = 1, 2, \dots, n.
% \end{equation}

% The chain rule allows us to compute the gradients efficiently, even for complex functions with multiple layers of dependencies. Consider $f(\boldsymbol{x})$ to be a simulation workflow where $\boldsymbol{x}$ are the geometry parameters that are subject to optimization and $y = f(\boldsymbol{x})$ the output of the simulation. By using a cost function $\mathcal{L}$ and applying the chain rule, the gradient of the cost function can be split into different parts that can be treated individually

% \begin{align}
%     \frac{\partial \mathcal{L}}{\partial \boldsymbol{x}} = \frac{\partial \mathcal{L}}{\partial f_\text{Postprocessing}} \frac{\partial f_\text{Postprocessing}}{\partial f_\text{Simulation}} \frac{\partial f_\text{Simulation}}{\partial f_\text{Geometry shape}} \frac{\partial f_\text{Geometry shape}}{\partial \boldsymbol{x}}.
% \end{align}
% Given analytical expressions for the loss function, the post-processing and the parametrization of the geometry shape, it remains to derive an expression for the derivative of the simulation with respect to the geometrical shape. In the following, we will apply the adjoint method to compute the derivative of the simulation with respect to the geometry shape and integrate the computation into a backpropagation framework to handle the computation of gradients. 

% \subsection{The adjoint method}
% The adjoint method is a powerful technique for sensitivity analysis of systems that are governed by partial differential equations (PDEs) which are too complicated to be solved analytically. Here we want to present a brief derivation of the idea following \cite{Johnson_notes_on_adjoint_methods} but a thorough derivation can be found in \cite{Johnson_notes_on_adjoint_methods, Cao_adjoint_sensitivity_analysis}.\\
% Consider a linear system of equations 
% \begin{align}
%     A\bold{u} = \bold{b}    
% \end{align}
% where $A$ represents the system dynamics, $\bold{u}$ the solution to the problem and $\bold{b}$ the source terms and $A$ and $\bold{b}$ depend on a set of parameters $p$. The solution $\bold{u}$ is computed by solving
% \begin{align}
%     \bold{u} = A^{-1}\bold{b}.
% \end{align}
% The solution is evaluated by a function $f(\bold{u})$. Now, we are interested in the gradient of the loss function wrt. to the parameters $\frac{\p f}{\p p}$. By taking the derivative of the linear system of equations wrt. to $p$ and applying the chain rule we obtain
% \begin{align}
%     \frac{\p f}{\p p } = \left(\frac{\p f}{\p \bold{u}} A^{-1} \right) \left( \frac{\p \bold{b}}{\p p} - \frac{\p A}{\p p} \bold{u} \right) \stackrel{!}{=} \langle \bold{v} \vert \bold{u} \rangle.
% \end{align}
% The product on the left can be identified with the \textit{adjoint problem} 
% \begin{align}
%     A^\dagger \bold{v} = \frac{\p f}{\p \bold{u}}^\dagger
% \end{align}
% while the term on the right contains the solution of the \textit{forward problem} and the sensitivities of the source and the system dynamics. The derivative of the loss function can be computed by a vector-jacobian product also known as backward mode differentiation. This means that we can compute the gradient of arbitrary many parameters by solving two PDEs, the forward and the adjoint problem of the system. 


% \subsection{Shape calculus}
% Shape calculus deals with computing how to deform boundaries and geometries in order to obtain a shape gradient that can deform a geometry continuously to increase the value of a loss functional \cite{Harbrecht_shape_optimization, Hansen:15, lebbe_phd:19}. 
% Consider a domain $\dom$ which contains a subdomain $\Omega$ with a boundary denoted by $\p \Omega$. Following \cite{lebbe_phd:19}, we are interested in a shape perturbation $\delta \Omega$ that will increase (or decrease) a loss functional $\mathcal{J}(\Omega)$ defined by an integral over the domain $\dom$ and the external and internal boundaries of the domain of the solution to the PDE which describe the pyhsics of our problem. The solution $\bold{u}_\Omega$ depends on the shape of the subdomain $\Omega$
% \begin{align}
%     \mathcal{J}_\dom(\Omega) = \int_\dom f(u_\Omega(x)) \dx; \hspace{.5cm}  \mathcal{J}_{\p \Omega} (\Omega)= \int_{\p \dom} g(u_\Omega(\s))\ds 
% \end{align}
% The shape derivatives of the domain-dependent functional for the perturbations $\delta\Omega$ are given by \cite{lebbe_phd:19}
% \begin{align}
%     \frac{\d \mathcal{J}_\dom}{\d \,\delta\Omega}\,(\delta\Omega) &= \int_{\p \Omega} \delta\Omega\, \bold{\hat{n}} \, f(s) \, \ds + \int_\Omega\mathring{f}(\delta\Omega)\dx\\
%     \frac{\d \mathcal{J}_{\p \Omega}}{\d \,\delta\Omega}\,(\delta\Omega) &
%     = \int_{\p \Omega} \delta\Omega \, \bold{\hat{n}} \, \Bigl( \nabla g(s) \bold{\hat{n}} + \kappa g(s) \Bigr)  \ds + \int_{\delta \Omega} \mathring{g}(\delta \Omega) \ds
% \end{align}
% where $\bold{\hat{n}}$ denotes the surface normal on $\p\Omega$, $\kappa = \nabla \bold{\hat{n}}$ is the curvature of the surface, $\mathring{\cdot}$ denotes the material derivative and $\frac{\d \mathcal{J}}{\d \Omega}$ denotes the Fréchet derivative. As the derivatives suggest, the sensitivity of the loss functional $\mathcal{J}$ only depends on the normal component of the deformable domain surface, which is also known as the structure theorem \cite{Delfour:11_book_shape_and_geometries, lebbe_phd:19}(see II.1.1.3). The shape gradient is given by a scalar field $V_\Omega(s)$, the \textit{sensitivity field}
% \begin{align}
%     \frac{\d \mathcal{J}}{\d \,\delta\Omega}(\delta\Omega) = \int_{\p \Omega} \delta\Omega \, \bold{\hat{n}} \, V_\Omega(s)\d s = \int_{\p \Omega} \delta\Omega \, \bold{\hat{n}} (c_1 - c_2) u_\Omega v_\Omega \ds.
% \end{align}
% The values $c_1$ and $c_2$ incorporate the boundary conditions and changes of the solution on the boundary of $\Omega$ while $u_\Omega$ is the solution of the forward problem and $v_\Omega$ is the solution of the adjoint problem. For a gradient descent algorithm, the descent direction is then given by 
% \begin{align}
%     \delta\Omega = - V_\Omega(s) \, \bold{\hat{n}}
% \end{align} 
% which assures a decrease of the functional to first order. The sensitivity field $V_\Omega(s)$ depends on the chosen functional and the function $f$ or $g$. Particularly the function $\nabla g$ depends on the derivative of the solution of the PDE. Then, the sensitivity field evaluated on the surface of the deformable boundary in the direction of the surface normal is the expression we need to obtain the derivative of the simulation with respect to the geometry shape
% \begin{align}
%     \frac{\partial f_\text{Simulation}}{\partial f_\text{Geometry shape}} = - V_\Omega(s) \bold{\hat{n}}.
% \end{align}

% \subsection{Adjoint method for photonics problems}
% By explicitly introducing the Maxwell equations into the problem, the sensitivity field for photonic shape optimization can be derived \cite{lebbe_phd:19, Hansen:15, Miller:13-Adjoint_shape_optimization}. 
% \begin{align}
%     Au_\Omega = 
%     \begin{pmatrix}
%     0   &   0   &   \nabla  &   0 \\
%     0   &   0   &   -\p t  & \nabla\times \\
%     \nabla\times    &   \p_t    &   0   &   0   \\
%     0   &   \nabla  &   0   &   0   \\
%     \end{pmatrix}
%     \begin{pmatrix}
%         E\\
%         B\\
%         D\\
%         H\\
%     \end{pmatrix}_\Omega = 
%     \begin{pmatrix}
%         j\\
%         m\\
%         0\\
%         0\\
%     \end{pmatrix} = b
% \end{align}
% where $j$ and $m$ denote the electric and magnetic source terms and $D=\varepsilon E$ and $H = \mu B$ are the electric and magnetic displacement fields inside a given material. We consider time-harmonic fields, ie, the solutions to the electric and the magnetic fields are given by $E(\x,t) = E_0(\x) e^{-i\omega t}$ and $H(\x,t) = H_0(\x)e^{-i\omega t}$. The solution will be computed via the numeric FDTD solver Lumerical and the solution of the time domain run is then Fourier transformed. 
% The sensitivity field at a boundary is given by
% \begin{align}
%     V_\Omega = \text{Re} \left[ (n^2_\text{in}-n^2_\text{out}) E_\parallel E^\dagger_\parallel - \left(\frac{1}{n^2_\text{in}}-\frac{1}{n^2_\text{out}}\right) E_\perp E^\dagger_\perp \right]
% \end{align}
% where $n_\text{in}$ and $n_\text{out}$ denote the refractive index on the inside and on the outside of the boundary where which are defined by the direction of the surface normal $\bold{\hat{n}}$.

% The adjoint problem of the Maxwell equations has the nice property $A = T A^\dagger T$ where $T$ is the time reversal operator \cite{Hansen:15}. This means that we can use the same solver without the need to change the update equations in the FDTD code by applying the time reversal to the adjoint source term $\frac{\p \mathcal{L}}{\p u_\Omega}$, finding the solution for the adjoint problem and again applying time reversal to receive $E^\dagger$.  

% \subsection{Combining the adjoint method and shape calculus into backpropagation}
% \todo[inline]{This paper or next paper?}
% Computing analytical derivatives for complicated physics problems with many post-processing steps and a complex geometrical model involves tedious and time-consuming work. Autodifferentiation is particularly useful since it involves computing analytical derivatives only for atomic steps in the computation of a complicated function. As we have seen, the derivation of the adjoint method enables us to identify the step where we can insert the adjoint method naturally into autodifferentiation for which we provide some pseudocode in \ref{algo:differentiable_simulation}. 
% We can create a \textit{differentiable simulation} by defining the forward method of such an autodifferentiation function to take the (discretized) set of the shape which is up for optimization and return the solution of the simulation as well as store the shape and the simulation result since we need it to compute the backward pass. In the backward pass, backpropagation through the computational graph returns the \textit{gradient input} for the differentiable simulation which is precisely the adjoint source term $\frac{\p \mathcal{L}}{\p u_\Omega}$. The backward method of the differentiable simulation then starts the simulation with the adjoint source term and receives the adjoint solution from the solver. Then, it computes the sensitivity field and evaluates the sensitivity field on the shape which are returned and passed by the computational graph to the next backward method.  



% % The adjoint method is a powerful technique for sensitivity analysis in nanophotonic structures, which enables the efficient computation of gradients in complex photonic systems. The method is based on the concept of the adjoint problem, which is derived from the original problem by transposing the governing equations and reversing the direction of time.

% % Consider a linear time-domain system governed by the equation $A\boldsymbol{E} = \boldsymbol{b}$, where $\boldsymbol{E}$ represents the electric field, $A$ is the linear operator, and $\boldsymbol{b}$ is the source term. The objective is to compute the sensitivity of a scalar quantity $F$ with respect to a parameter $p$, given by $\frac{\partial F}{\partial p}$. 

% % The adjoint problem is defined as $A^T\boldsymbol{E}^* = \boldsymbol{b}^*$, where $A^T$ is the transpose of $A$, and $\boldsymbol{E}^*$ and $\boldsymbol{b}^*$ are the adjoint field and source, respectively. The adjoint source $\boldsymbol{b}^*$ is chosen such that the inner product of the adjoint field $\boldsymbol{E}^*$ with the derivative of the source term $\frac{\partial \boldsymbol{b}}{\partial p}$ is equal to the sensitivity of the scalar quantity $F$ with respect to the parameter $p$:

% % \begin{equation}
% % \frac{\partial F}{\partial p} = \left<\boldsymbol{E}^*, \frac{\partial \boldsymbol{b}}{\partial p} \right>.
% % \end{equation}

% % \subsection{Shape gradients in adjoint method}

% % To derive the shape gradients from the adjoint method, we follow the approach presented in Paul Hansen's work. The shape gradient is given by the derivative of the objective functional $J$ with respect to the shape parameter $s$:

% % \begin{equation}
% % \frac{dJ}{ds} = \left<\boldsymbol{E}^*, \frac{\partial \boldsymbol{b}}{\partial s} \right> - \left<\boldsymbol{E}, \frac{\partial A^T \boldsymbol{E}^*}{\partial s} \right>.
% % \end{equation}

% % The first term in the equation represents the contribution of the change in the source term with respect to the shape parameter, while the second term represents the contribution of the change in the adjoint field due to the shape variations.

% % By computing the shape gradients, we can update the structure iteratively to optimize the performance of the photonic device. The adjoint method allows for the efficient computation of gradients in complex photonic systems, providing a powerful tool for the optimization of nanophotonic structures, including µLED outcoupling structures.



